Efficient and Scalable MIV-transistor with Extended Gate in Monolithic 3D Integration

Monolithic 3D integration has become a promising solution for future computing needs. The metal inter-layer via (MIV) forms interconnects between substrate layers in Monolithic 3D integration. Despite small size of MIV, the area overhead can become a major limitation for efficient M3D integration and, thus needs to be addressed. Previous works focused on the utilization of the substrate area around MIV to reduce this area overhead significantly but suffers from increased leakage and scaling factors. In this work, we discuss MIV-transistor realization that addresses both leakage and scaling issue along with similar area overhead reduction compared with previous works and, thus can be utilized efficiently. Our simulation results suggest that the leakage current $(I_{D,leak})$ has reduced by $14K\times$ and, the maximum current $(I_{D,max})$ increased by $58\%$ for the proposed MIV-transistor compared with the previous implementation. In addition, performance metrics of the inverter realization with our proposed MIV-transistor specifically the delay, slew time and power consumption reduced by $11.6\%$, $17.9\%$ and, $4.5\%$ respectively compared with the previous implementation with same MIV area overhead reduction.

==> Section_Previous_models.tex <==
\section{Pitfalls in previous work}\label{sec:previous_work}
 
 \begin{figure}
     \centering
     \includegraphics[width=\linewidth]{Figures/simulations/varying.png}
     \caption{Caption}
     \label{fig:my_label}
 \end{figure}

